On some Operator Filtering Strategies Based on Suitably Modified Green's Functions

Recent contributions showed the benefits of operator filtering for both preconditioning and fast solution strategies. While previous contributions leveraged laplacian-based filters, in this work we introduce and study a different approach leveraging the truncation of appropriately chosen spectral representations of operators' kernels. In this contribution, the technique is applied to the operators of the 2D TE- and TM-electric field integral equations (EFIE). We explore two different spectral representations for the 2D Green's function that lead to two distinct types of filtering of the EFIE operators. Numerical results corroborate the effectiveness of the newly proposed approaches, also in the Calder\'on preconditioned EFIE

==> definitions.tex <==
%%% highlight
\newcommand{\hlr}[1]{\sethlcolor{red}\hl{#1}}
\newcommand{\hlg}[1]{\sethlcolor{green}\hl{#1}}
\newcommand{\hlo}[1]{\sethlcolor{orange}\hl{#1}}

%%% math
\newcommand\bs[1]{\boldsymbol{#1}} %vector
\newcommand\mbf[1]{\mathbf{#1}} %algebraic vector
\newcommand\bsh[1]{\hat{\boldsymbol{#1}}} %versor vector
\newcommand\mbb[1]{\mathbb{#1}} %auto math \mathbb 
\newcommand\mcal[1]{\mathcal{#1}}
\newcommand\diam[1]{\mathbf{#1}^\diamond}
\newcommand\bull[1]{\mathbf{#1}^\bullet}

%%% specialized definitions (most used)
\newcommand\thetah{\bs{\hat{\theta}}}
\newcommand\phih{\bs{\hat{\phi}}}
\newcommand\x{\bs{x}}
\newcommand\xp{\bs{x}^\prime}
\newcommand\Ps{\mbf{P}^\Sigma}
\newcommand\Psh{\mbf{P}^\Sigma H}
\newcommand\Pl{\mbf{P}^\Lambda}
\newcommand\Plh{\mbf{P}^{\Lambda H}}
\newcommand\G{\mbf{G}}
\newcommand\Lam{\mbf{\Lambda}}
\newcommand\Sig{\mbf{\Sigma}}
\newcommand\Pc{\mcal{P}}
\newcommand\Ic{\mcal{I}}
\newcommand\Kc{\mcal{K}}
\newcommand\Tc{\mcal{T}}
\newcommand\Sc{\mcal{S}}


%%% more math
\newcommand\im{\mathrm{i}\mkern 1mu}
\newcommand\lrr[1]{\left(#1\right)}
\newcommand\lrs[1]{\left[#1\right]}
\newcommand\lrc[1]{\left\{#1\right\}}
\newcommand\lrw[1]{\big|#1\big|}
\newcommand\lra[1]{\langle#1\rangle} \newcommand\Lra[1]{\Big\langle#1\Big\rangle}
\newcommand\RE[1]{\operatorname{Re}\lrc{#1}}
\newcommand\IM[1]{\operatorname{Im}\lrc{#1}}
\newcommand\diff{\mathrm{d}}
\newcommand\grad{\nabla}
\newcommand\diver{\nabla\cdot}
\newcommand\rot{\nabla\times}
\newcommand\divers{\nabla_s\cdot}
\newcommand\parz[2]{\frac{\partial{#1}}{\partial{#2}}}
\newcommand\parzm[3]{\frac{\partial^{#3}{#1}}{\partial{#2}^{#3}}}
\newcommand\differ[2]{\frac{\diff#1}{\diff#2}}
\newcommand\differm[3]{\frac{\diff^{#3}#1}{\diff{#2}^{#3}}}

%%% physics
\newcommand\nh{\hat{\bs{n}}}
\newcommand\nt{\tilde{\bs{n}}}
\newcommand\rh{\hat{\bs{r}}}
\newcommand\ix{\mbf{i}_x}
\newcommand\iy{\mbf{i}_y}
\newcommand\iz{\mbf{i}_z}
\newcommand\Zinf{Z_\infty}
\newcommand\Yinf{Y_\infty}
\newcommand\w{\omega}

%%% language
\newcommand\cald{Calder\'{o}n }

%%% macros
\newcommand{\td}[1]{\todo[inline]{#1}}


==> title_singleColumn_URSI.tex <==
\makeatletter

\newcounter{author}
\renewcommand{\author}[2][]{
   \stepcounter{author}
   \@namedef{author@\theauthor}{#2}
   \@namedef{authorlabel@\theauthor}{#1}
}

\newcounter{address}
\newcommand{\address}[2][]{
   \stepcounter{address}
   \@namedef{address@\theaddress}{#2}
   \@namedef{addresslabel@\theaddress}{#1}
}

\newcommand{\alsep}{and}

% this is borrowed from IEEEtran.cls and revised for single column author block formatting
\def\newmaketitle{\par%
  \begingroup%
  \normalfont%
  \def\thefootnote{}%  the \thanks{} mark type is empty
  \def\footnotemark{}% and kill space from \thanks within author
  \let\@makefnmark\relax% V1.7, must *really* kill footnotemark to remove all \textsuperscript spacing as well.
  \footnotesize%       equal spacing between thanks lines
  \footnotesep 0.7\baselineskip%see global setting of \footnotesep for more info
  \normalsize%
  \twocolumn[\thenewmaketitle\@IEEEaftertitletext]%
  % pullup page for pubid if used.
  \if@IEEEusingpubid
     \enlargethispage{-\@IEEEpubidpullup}%
  \fi
  \endgroup
  \setcounter{footnote}{0}\let\maketitle\relax\let\@maketitle\relax
  \gdef\@thanks{}%
  % v1.6b do not clear these as we will need the title again for peer review papers
  % \gdef\@author{}\gdef\@title{}%
  \let\thanks\relax}

% this is borrowed from ursi2022.cls for single column author block formatting
\def\thenewmaketitle{
% Add the formatted title
  \newpage
  \begin{center}%
    \vskip0.2em{\Huge\@IEEEcompsoconly{\sffamily}\@IEEEcompsocconfonly{\normalfont\normalsize\vskip 2\@IEEEnormalsizeunitybaselineskip
   \bfseries\large}\@title\par}\vskip1.0em\par%
   %
    \vspace{1ex}
    \newcounter{c@author}
    \newcounter{c@tmp}
    \ifthenelse{\value{author}=2}{%
      \newcommand{\liand}{ and }}{%
      \newcommand{\liand}{, and }}
    % Next add the authors
    \ifthenelse{\value{address}<2}{%
      %No address references required if there is only one
      \@nameuse{author@1}%
      \stepcounter{c@author}%
      \whiledo{\value{c@author}<\value{author}}{%
        \setcounter{c@tmp}{\value{author}}%
        \addtocounter{c@tmp}{-\value{c@author}}%
        \ifthenelse{\value{c@tmp}=1}{%
          \renewcommand{\alsep}{\liand}}{\renewcommand{\alsep}{, }}%
        \stepcounter{c@author}\alsep \@nameuse{author@\thec@author}}\\%
    }
    {%Add address references after the author's name
      \@nameuse{author@1}${}^{(\ref{\@nameuse{authorlabel@1}})}$%
      \stepcounter{c@author}%
      \whiledo{\value{c@author}<\value{author}}{%
      \setcounter{c@tmp}{\value{author}}%
      \addtocounter{c@tmp}{-\value{c@author}}%
      \ifthenelse{\value{c@tmp}=1}{%
        \renewcommand{\alsep}{\liand}}{\renewcommand{\alsep}{, }}%
      \stepcounter{c@author}\alsep \@nameuse{author@\thec@author}%
        ${}^{(\ref{\@nameuse{authorlabel@\thec@author}})}$%
      }
    }
%    \theaddress
    \vspace{0.2ex}

    \ifthenelse{\value{address}>0}{%
      \ifthenelse{\value{address}=1}{
        %Output the address without any reference symbols
       %%        {\slshape\small \@nameuse{address@1}}
        {\@nameuse{address@1}}
      }
      {%Output the addresses as an enumerated list
        \newcounter{c@address}

        \begin{center}
        \whiledo{\value{c@address}<\value{address}}
        {
          \refstepcounter{c@address}
            ${}^{(\thec@address)}$\,%
              \label{\@nameuse{addresslabel@\thec@address}}%
              \@nameuse{address@\thec@address}\\ %
        }
        \end{center}
      } % end of the address creation ifthenelse block
    }
    {
      \relax
    }
  \end{center}
}

\makeatother

%FROM HERE ON, THIS IS A TEMPLATE FOR THE MAIN LATEX DOCUMENT

% paper title
% can use linebreaks \\ within to get better formatting as desired
%\title{A new class of filtered operators}

% authors and affiliations
% the organization option [orgN] associates the authors with the
% proper address
%\author[org1]{Matteo E. Masciocchi}
%\author[org1]{Ermanno Citraro}
%\author[org2]{Alex}

% each address must have a unique identifier in the option field
%\address[org1]{Department of Electronics and Telecommunications(DET), Politecnico di Torino, 10129 Turin, Italy}
%\address[org2]{The Next Company, Neverland, WA 54321, USA (author@next.com)}


%\begin{document}

%\newmaketitle

